Faster algorithms for circuits in the Cayley-Menger algebraic matroid

A classical problem in Distance Geometry, with multiple practical applications (in molecular structure determination, sensor network localization etc.) is to find the possible placements of the vertices of a graph with given edge lengths. For minimally rigid graphs, the double-exponential Gr\"obner Bases algorithm with an elimination order can be applied, in theory, but it is impractical even for small instances. By relating the problem to the computation of circuit polynomials in the Cayley-Menger ideal, we recently proposed an algebraic-combinatorial approach and an elimination algorithm for circuit polynomials [23]. It is guided by a tree structure whose leaves correspond to complete $K_4$ graphs and whose nodes perform algebraic resultant operations. In this paper we uncover further combinatorial structure in the Cayley-Menger algebraic matroid that leads to an extension of our algorithm. In particular, we generalize the combinatorial resultant operation of [23] to take advantage of the non-circuit generators and irreducible polynomials in the Cayley-Menger ideal and use them as leaves of the tree guiding the elimination. Our new method has been implemented in Mathematica and allows previously unobtainable calculations to be carried out. In particular, the $K_{3,3}$-plus-one circuit polynomial, with over one million terms in 10 variables and whose calculation crashed after several days with the previous method of [23], succeeded now in approx. 30 minutes.

==> combResCircuits.tex <==
\section{Combinatorial Resultant Constructions.}
\label{sec:combRes}

We define now a new operation, the \emph{combinatorial resultant} of two graphs, prove \cref{thm:combResConstruction} and describe its algorithmic implications. 

\subsection{Definition: Combinatorial resultant.}
	Let $G_1$ and $G_2$ be two distinct graphs with non-empty intersection $E_{\cap} \neq\emptyset$ and let $e\in E_{\cap}$ be a common edge. The {\em combinatorial resultant} of $G_1$ and $G_2$ on the {\em elimination edge} $e$ is the graph $\cres{G_1}{G_2}{e}$ with vertex set $V_{\cup}$ and edge set $E_{\cup}\setminus\{e\}$.

\begin{figure}[ht]
	\centering
	% \includegraphics[width=0.18\textwidth]{New/k4.pdf}
	% \includegraphics[width=0.22\textwidth]{New/w4.pdf}
	% \includegraphics[width=0.27\textwidth]{New/common.pdf}
	% \includegraphics[width=0.27\textwidth]{New/cres.pdf}
	\caption{A complete $K_4$ graph, a $4$-wheel $W_4$, their common edges (dotted, with elimination edge in red) and their combinatorial resultant, which has more than $2n-2$ edges and thus is not a circuit.}
	\label{fig:graphK4W4}
\end{figure}

The 2-sum appears as a special case of a combinatorial resultant when the two graphs have exactly one edge in common, which is eliminated by the operation. Circuits are closed under the $2$-sum operation, but they are not closed under this general combinatorial resultant operation: two examples is shown in \cref{fig:graphK4W4} and \cref{fig:graphW5K4}. 

\begin{figure}[ht]
	\centering
	% \includegraphics[width=0.24\textwidth]{w4-in-wheel.pdf}
	% \includegraphics[width=0.24\textwidth]{k4-in-w4.pdf}
	% \includegraphics[width=0.24\textwidth]{laman-common.pdf}
	% \includegraphics[width=0.24\textwidth]{laman-plus-one.pdf}	
	\caption{A $4$-wheel $W_4$, a complete $K_4$ graph,  their common  Laman graph (dotted, with red elimination edge) and their combinatorial resultant, which is a Laman-plus-one graph but not a circuit.}
	\label{fig:graphW5K4}
\end{figure}

\subparagraph{Circuit-valid combinatorial resultants.} We are interested in combinatorial resultants that produce circuits from circuits. Towards this goal, we say that two circuits are {\em properly intersecting} if their common subgraph (of common vertices and common edges) is Laman. The example in \cref{fig:graphK4W4} is not properly intersecting, but those in \cref{fig:graphW5K4} and \cref{fig:combResultant} are.

\begin{lemma}
	\label{lem:combRes2n2}
	The combinatorial resultant of two circuits has $m=2n-2$ edges iff the common subgraph $G_{\cap}$ of the two circuits is Laman.
\end{lemma}



\begin{figure}[ht]
	\centering
	% \includegraphics[width=0.24\textwidth]{w4.pdf}
	% \hspace{-40pt}
	% \includegraphics[width=0.24\textwidth]{k4.pdf}
	% \includegraphics[width=0.24\textwidth]{common.pdf}
	% \includegraphics[width=0.24\textwidth]{w5.pdf}
	\caption{A $4$-wheel $W_4$ and a complete $K_4$ graph, their common  Laman graph (dotted, with red elimination edge) and their combinatorial resultant, the $5$-wheel $W_5$ circuit.}
	\label{fig:combResultant}
\end{figure}

\begin{proof} 
Let $C_1$ and $C_2$ be two circuits with $n_i$ vertices and $m_i$ edges, $i=1,2$, and let $C$ be their combinatorial resultant with $n$ vertices and $m$ edges.
By inclusion-exclusion $n=n_1+n_2-n_{\cap}$ and $ m = m_1 + m_2 - m_{\cap} - 1$.
% , where $n_{\cap} = |V_{\cap}|$ and $m_{\cap} = |E_{\cap}|$.
Substituting here the values for $m_1=2n_1-2$ and $m_2=2n_2-2$, we get $ m = 2 n_1 - 2 + 2 n_2 - 2 - m_{\cap} - 1 = 2(n_1 + n_2 - n_{\cap}) -2 + 2 n_{\cap} - 3 - m_{\cap} = (2n-2) + (2 n_{\cap} - 3) - m_{\cap}$. We have $m = 2 n -2$ iff $m_{\cap} = 2 n_{\cap} - 3$. Since both $C_1$ and $C_2$ are circuits, it is not possible that one edge set be included in the other: circuits are minimally dependent sets of edges and thus cannot contain other circuits. As a proper subset of both $E_1=E(C_1)$ and $E_2=E(C_2)$, $E_{\cap}$  satisfies the hereditary $(2,3)$-sparsity property. If furthermore $G_{\cap}$ has exactly $2 n_{\cap} - 3$ edges, then it is Laman.
\end{proof}

It is important to retain that the {\em common subgraph} is defined on both the common vertex and the common edge set. The following lemma allows us to sometimes consider just the graph {\em induced on the common vertex set} in the union of $G_1$ and $G_2$, when checking if two circuits are properly intersecting. This observation is applicable to the type of combinatorial resultants used from now on in this paper.
 
\begin{lemma}
	\label{lem:combResCommon}
	Let $C_1 = (V_1, E_1)$ and $C_2 =(V_2, E_2)$ be two circuits whose common vertex set $V_{\cap}$ is a strict subset of both $V_1$ and $V_2$. If the common subgraph $G_{\cap}=(V_{\cap},E_{\cap})$ is Laman, then neither $C_1$ nor $C_2$ contain additional edges (besides $E_{\cap}$) spanned by their common vertices.
\end{lemma}

\begin{proof} 
	Assume that $C_1$ contains an additional edge spanned by $V_{\cap}$. Since $(V_{\cap},E_{\cap})$ is Laman, this edge induces a circuit, entirely contained in $C_1$ and spanned by a proper subset of the vertices of $V_1$: this contradicts the fact that $C_1$ is a circuit: by the definition of a circuit, as a minimal dependent set of edges, a circuit cannot contain a subgraph that is smaller, yet dependent.
\end{proof}


\noindent
A combinatorial resultant operation applied to two properly intersecting circuits is said to be \emph{circuit-valid} if it results in a spanning circuit. An example is shown in \cref{fig:combResultant}. Being properly intersecting is a necessary condition for the combinatorial resultant of two circuits to produce a circuit, but the example in \cref{fig:graphW5K4} shows that this is not sufficient. 

\begin{problem}
Find necessary and sufficient conditions for the combinatorial resultant of two circuits to be a circuit.
\end{problem}


Our first goal is to show that each circuit can be obtained from $K_4$ circuits via a sequence of circuit-valid combinatorial resultant operations, in a manner that adds at least one new vertex at each step.

\subsection{Proof of \cref{thm:combResConstruction}.}
\label{ssec:proofThm1}

We prove now that each rigidity circuit can be obtained, inductively, by applying combinatorial resultant operations starting from $K_4$ circuits. The proof handles separately the $2$- and $3$-connected cases. In \cref{sec:prelimRigidity} we have seen that a $2$-connected circuit can be obtained from $3$-connected circuits via $2$-sums. The bulk of the proof is in the following proposition, which handles the $3$-connected circuits.

\begin{proposition}
	\label{prop:circuits3conn}
	Let $C=(V,E)$ be a $3$-connected circuit spanning $n+1\geq 5$ vertices. Then, in polynomial time, we can find two circuits $A$ and $B$ such that $A$ has $n$ vertices, $B$ has at most $n$ vertices and $C$ can be represented as the combinatorial resultant of $A$ and $B$.
\end{proposition}

\begin{proof}
We apply a weaker version of \cref{thm:BergJordan} to find two non-adjacent vertices $a$ and $b$ of degree 3 such that a circuit $A=(V\setminus{\{a\}},E\setminus{\{au,av,aw\}})$ can be produced via an inverse Henneberg II operation on vertex $a$ in $C$ (see \cref{fig:invCombResA}). Let the neighbors of vertex $a$ be $N(a)=\{u,v,w\}$ such that $e=uw$ was not an edge of $C$ and is the one added to obtain the new circuit $A$. 
%
\begin{figure}[ht]
	\centering
		% \includegraphics[width=.34\textwidth]{initCircuitC.pdf}
		% \includegraphics[width=.31\textwidth]{invHennOnA.pdf}
		% \includegraphics[width=.3\textwidth]{circuitA.pdf}
	\caption{
	The 3-connected circuit $C$ spanning $n+1$ vertices with two non-adjacent vertices $a$ (red) and $b$ (blue) of degree 3. Note that $N(a)$ and $N(b)$ may not be disjoint. An inverse Henneberg II at $a$ removes the red edges at $a$ and adds dotted red edge $e = uv$. Circuit $A$ (red). 
	}
	\label{fig:invCombResA}
\end{figure}
%
To define circuit $B$, we first let $L$ be the subgraph of $C$ induced by $V\setminus\{b\}$. Simple sparsity consideration show that $L$ is a Laman graph. The graph $D$ obtained from $L$ by adding the edge $e=uv$, as in \cref{fig:invCombResB} (left), is a Laman-plus-one graph 
% (not necessarily a spanning circuit)
containing the three edges incident to $a$ (which are not in $A$) and the edge $e$ (which is in $A$). $D$ contains a unique circuit $B$ (\cref{fig:invCombResB} left) with edge $e\in B$ (see e.g.~\cite[Proposition 1.1.6]{Oxley:2011}). It remains to prove that $B$ contains $a$ and its three incident edges. If $B$ does not contain $a$, then it is a proper subgraph of $A$. But this contradicts the minimality of $A$ as a circuit. Therefore $a$ is a vertex in $B$, and because a vertex in a circuit can not have degree less than $3$, $B$ contains all its three incident edges.

\begin{figure}[ht]
	\centering
		% \includegraphics[width=.33\textwidth]{deleteB.pdf}
		% \includegraphics[width=.3\textwidth]{circuitB.pdf}
	\caption{
	Remove from $C$ the edges from $b$ (blue dotted) and add red edge $e$. Circuit $B$ (blue).}
	\label{fig:invCombResB}
\end{figure}

The combinatorial resultant $\cres{A}{B}{e}$ of the circuits $A$ and $B$ with $e$ the eliminated edge satisfies the desired property that $C=\cres{A}{B}{e}$.
\end{proof}

\subsection{Algorithmic aspects.} The algorithm below captures the procedure described in \cref{prop:circuits3conn}. It can be applied recursively until the base case $K_4$ is attained.  Its main steps, the Inverse Henneberg II step on a circuit at line \ref{line:invH} and finding the unique circuit in a Laman-plus-one graph at line \ref{line:circuit} can be carried out in polynomial time using slight variations of the $(2,3)$ and $(2,2)$-sparsity pebble games from \cite{streinu:lee:pebbleGames:2008}.  


\begin{algorithm}[ht]
	\caption{Inverse Combinatorial Resultant}
	\label{alg:comb}
	\textbf{Input}: $3$-connected circuit $C$\\
	\textbf{Output}: circuits $A$, $B$ and edge $e$ such that $C=\cres{A}{B}{e}$
	\begin{algorithmic}[1]
		\For{each vertex $a$ of degree $3$}
		\If{inverse Henneberg II is possible on $a$\\ \ \ \ \ \textbf{and} there is a non-adjacent degree $3$  vertex $b$}
		\State Get the circuit $A$ and the edge $e$ by inverse Henneberg II in $C$ on $a$\label{line:invH}
		\State Let $D = C$ without $b$ (and its edges) and with new edge $e$
		\State Compute the unique circuit $B$ in $D$ \label{line:circuit}
		\State \Return circuits $A, B$ and edge $e$
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}

The algorithm faces many choices for the two degree-$3$ vertices $a$ and $b$. These choices may lead to different representations of a circuit as the combinatorial resultant of two other circuits. 

\begin{corollary}\label{cor:nonunique}
The representation of $C$ as the combinatorial resultant of two smaller circuits is in general not unique. An example is the ``double-banana'' 2-connected circuit shown in \cref{fig:exampleCircuit}.
\end{corollary}

\begin{figure}[ht]
\centering
% \includegraphics[width=.3\textwidth]{doubleBanana1.pdf}
% \includegraphics[width=.3\textwidth]{doubleBanana2.pdf}
\caption{The 2-connected {\em double-banana} circuit can be obtained as a combinatorial resultant from two $K_4$ graphs (left, $2$-sum), and from two wheels on 4 vertices sharing two triangles (right). Dashed lines indicate the eliminated edges, and in each case one of the two circuits is highlighted to distinguish $K_4$ from $W_4$.}
\label{fig:exampleCircuit}
\end{figure}

\subsection{Combinatorial Resultant tree.}\label{sec:resultantTree} 
Each one of the possible constructions of a circuit using combinatorial resultant operations can be represented in a {\em tree} structure. Let $C$ be a rigidity circuit with $n$ vertices. A \emph{resultant tree} $T_C$ for the circuit $C$ is a rooted binary tree with $C$ as its root and such that: (a) the nodes of $T_C$ are circuits; (b) circuits on level $l$ have at most $n-l$ vertices; (c) the two children $\{C_j,C_k\}$ of a parent circuit $C_i$ are such that $C_i=\cres{C_j}{C_k}{e}$, for some common edge $e$, and (d) the leaves are complete graphs on 4 vertices. An example is illustrated in \cref{fig:resTree}.


\begin{figure}[ht]
	\centering
		% \includegraphics[width=.7\textwidth]{New/cresTree.pdf}
	\caption{
	A combinatorial resultant tree for the Desargues-plus-one circuit. To help the reader visualize the common Laman subgraphs and the eliminated edge at each node of the tree, the lower circuits are shown, in black and with large vertices, in the context of the combinatorial resultant circuit above them (light-greyed).}
	\label{fig:resTree}
\end{figure}


\subparagraph{Complexity of resultant trees.} If the intermediate circuits are all $3$-connected, the depth of a tree obtained by our method is $n-4$, and this is the worst possible case. The best case for depth is $\log n$ and occurs when all the intermediate circuits are $2$-connected and are split into two circuits of the same size.

In terms of size (number of nodes), the combinatorial resultant tree may be, in principle, anywhere between linear to exponential in size. Best cases occur when the resultant tree is path-like, with each internal node having a $K_4$ leaf, or when the tree is balanced of depth $\log n$ and each resultant operation is a $2$-sum. Conceivably, the worst case (exponential size) could be a complete (balanced) binary tree of linear depth: each internal node at level $k$ would combine two circuits with the same number of vertices $n-k-1$ into a circuit with $n-k$ vertices. Sporadic examples of small balanced combinatorial resultant trees exist (e.g. for $K_{33}$-plus-one), but we do not know how far they generalize.

%REQUEST: we'd like to have the open problems numbered consecutively and separately from theorems or remarks. Is it possible?

\begin{problem}
	Are there infinite families of circuits with linear-depth, balanced combinatorial resultant trees? 
\end{problem}


It would be interesting to understand the worst case size of these trees, even if families as above do not exist:

\begin{problem}
	Characterize the circuits produced by the worst-case size of the combinatorial resultant tree. 
\end{problem}

Understanding the worst cases may help our Algorithm \ref{alg:comb} avoid the corresponding choices of vertices $a$ and $b$ in Steps 1-3. The goal would then be to produce the {\em best resultant tree,} or at least a good one, according to some well-defined measure of {\em resultant tree complexity}. 


\subparagraph{Complexity measures for resultant trees.} Looking ahead to \cref{sec:algResCircuits}, we remark that the complexity of the algebraic part of our algorithm for computing circuit polynomials is influenced by several factors encoded in the resultant tree: the size of the tree (number of resultant operations),  its depth and the specificity of the elimination edge at each internal node. 

The {\em best} resultant tree could be defined in terms of a particular measure (size, depth, etc.), or some combination of them. 

\begin{problem}
	Define a meaningful measure of (combinatorial) resultant-tree complexity that would lead to effective computations of larger\footnote{E.g. larger than  those reported in  \cref{sec:experiments}.} circuit polynomials (cf. \cref{sec:algResCircuits}). 
\end{problem}

Such a complexity measure will affect the complexity of the optimization version of the {\em combinatorial resultant tree} problem based on Algorithm \ref{alg:comb}. The resulting tree would have a major influence on the practical feasability of the subsequent algebraic calculations for circuit polynomials. We remark that the concrete calculations reported later on in \cref{sec:experiments} of this paper were possible because our resultant trees were easy to select for optimality from a small set of possibilities. As the number $n$ of vertices becomes larger than $7$, the number of possible resultant trees grows fast. 

\begin{problem}
	Refine Algorithm \ref{alg:comb} (and its analysis) to produce an {\em optimal} resultant tree, according to a measure of resultant-tree complexity leading to efficient resultant-based calculations of circuit polynomials (as described further ahead in \cref{sec:algResCircuits}). 
\end{problem}



